Cooperation Speeds Surfing: Use Co-Bandit!

In this paper, we explore the benefit of cooperation in adversarial bandit settings. As a motivating example, we consider the problem of wireless network selection. Mobile devices are often required to choose the right network to associate with for optimal performance, which is non-trivial. The excellent theoretical properties of EXP3, a leading multi-armed bandit algorithm, suggest that it should work well for this type of problem. Yet, it performs poorly in practice. A major limitation is its slow rate of stabilization. Bandit-style algorithms perform better when global knowledge is available, i.e., when devices receive feedback about all networks after each selection. But, unfortunately, communicating full information to all devices is expensive. Therefore, we address the question of how much information is adequate to achieve better performance. We propose Co-Bandit, a novel cooperative bandit approach, that allows devices to occasionally share their observations and forward feedback received from neighbors; hence, feedback may be received with a delay. Devices perform network selection based on their own observation and feedback from neighbors. As such, they speed up each other's rate of learning. We prove that Co-Bandit is regret-minimizing and retains the convergence property of multiplicative weight update algorithms with full information. Through simulation, we show that a very small amount of information, even with a delay, is adequate to nudge each other to select the right network and yield significantly faster stabilization at the optimal state (about 630x faster than EXP3).

==> evaluation/otherListenProbability.tex <==
We vary the probability with which a device listens for broadcast messages, i.e., value of $p_l$.
% and study its effect on the state at which the algorithm stabilizes and its rate of stabilization. 
We also consider a more realistic approach where a time slot is divided into 5 sub-time slots of equal duration. During each sub-time slot, a device transmits with probability $\frac{1}{n}$, and otherwise listens with probability $\frac{2}{5}$. It also implies that all devices may not hear the same feedback during a time slot. For example, it can leverage some duty cycling protocol, such as the Birthday protocol, to decide whether to transmit, listen, or save energy. Figure \ref{figure:different_listen_probability_distanceToNashEquilibrium} shows that the distance increases as the value of $p_l$ drops and the performance is significantly better with the \enquote{realistic} approach. In the latter case, and when $p_l = 1$ or $0.75$, all runs stabilized at Nash equilibrium. When $p_l = 0.5$, 2 runs had a single device in the \enquote{wrong} network and 3 runs did not stabilize; in 2 of the 3 runs, there a reset near the end of the run when a device explored a network unheard of --- but, over 82\% time was spent at Nash equilibrium. In all cases, the algorithm is at least at $\epsilon$-equilibrium.
% run110 - device 7 reset at t = 1187 when exploring network 5 - original stable at network 3 (at the same time device 2 from network 5 was exploring network 2)
% run 223
% run 417 - same thing as in run 110 happened here with device 5 that reset at t - 1188

From Table \ref{table:different_listen_probability_cumulative_download_stabilization_rate}, we can see that the median cumulative gain of a device in all cases are comparable. The median time taken to stabilize (whether to Nash equilibrium or some other state) increases as the value of $p_l$ drops, and is lowest when the \enquote{realistic} approach is considered given that it increases the probability that a device receives feedback from its neighbors. In that case, it takes only about (median) 14\% more time to stabilize compared to EWA (as given in Table \ref{table:minimal_reset_cumulative_download_stabilization_rate}).

\begin{figure}[!htb]
\begin{center}
\includegraphics [scale=0.84]
{plot/different_listen_probability_distanceToNashEquilibrium.pdf}
\end{center}
\caption{Effect of different probability of listening on average distance to Nash equilibrium (\% higher gain any device would have observed, compared to its current gain, if the algorithm was at Nash equilibrium) --- shaded region represents $\epsilon$-equilibrium, where $\epsilon = 7.5$.}
\label{figure:different_listen_probability_distanceToNashEquilibrium}
\end{figure}

\input{table/different_listen_probability_cumulative_download_stabilization_rate}
% $p_l = 0.5$
% 495 runs stable at NE [2, 2, 7, 5, 4]
% 2 in a state that requires 1 to move [1, 2, 8, 5, 4], [1, 2, 7, 5, 5]
% 3 not stable

% others all 100\% stable at NE
\color{red} must re-run simulation without reset \color{black}

==> table/algorithm_comparison.tex <==
\begin{table}[!htb]
\small
\centering
\caption{Algorithms compared to  Co-Bandit.}
\label{table:algorithm_comparison}
\newcolumntype{L}{>{\arraybackslash}m{6.3cm}}
\begin{tabular}{c L}
\hline
% \textbf{Variable}    & \textbf{Description}                             \\ \hline
% EXP3     & Original EXP3 algorithm \cite{auer2002nonstochastic}.                
% \\ 
% \hline
EXP3 & It assigns a weight to each network. In each time slot, it selects a network at random based on a probability distribution that mixes between using the weights and a uniform distribution. At the end of a time slot, the device observes a gain (bit rate) from its chosen network and updates its weight using a multiplicative update rule \cite{auer2002nonstochastic}.
\\
\hline
Smart EXP3 & It maintains a weight for each network and uses the same weight and probability update rules as EXP3. However, it (a) starts by exploring each network in random order, (b) selects a network for a block (consecutive time slots) whose length increases with the frequency of selection of the network, (c) occasionally makes a deterministic (greedy) selection, (d) allows a device to switch back to its previous network upon selecting a worse network, and (e) performs a minimal reset periodically and when a significant drop is detected in the network being selected with sufficiently high probability. 
\\
\hline
\end{tabular}
\end{table}

==> table/different_listen_probability_cumulative_download_stabilization_rate.tex <==
\begin{table}[!htb]
\small
\centering
\caption{Effect of varying probability of listening on the median per device cumulative download (GB) and median number of slots taken to stabilize (whether at Nash equilibrium or some other state).}
\label{table:different_listen_probability_cumulative_download_stabilization_rate}
\newcolumntype{L}{>{\centering\arraybackslash}p{2.22cm}}
\begin{tabular}{c l L L L}
\hline
\textbf{\#sub-time slots} & \textbf{$p_l$} & \textbf{Cumulative download (GB)} & \textbf{\# time slots to stabilize} \\ \hline
\multicolumn{1}{l}{\textbf{1}} & \multicolumn{1}{l}{\textbf{1}} & 6.93 & 169 \\ 
% \hline
\multicolumn{1}{l}{\textbf{1}} & \multicolumn{1}{l}{\textbf{0.75}} & 6.93 & 185.5 \\ 
\multicolumn{1}{l}{\textbf{1}} &\multicolumn{1}{l}{\textbf{0.5}} & 6.91 & 290 \\
\multicolumn{1}{l}{\textbf{5}} &\multicolumn{1}{l}{\textbf{0.4}} & 6.95 & 104 \\ 
% \multicolumn{1}{l}{\textbf{5}} &\multicolumn{1}{l}{\textbf{0.4}} & 6.95 & 102 \\ 
\hline
\end{tabular}
\end{table}

==> table/minimal_reset_cumulative_download_stabilization_rate.tex <==
\begin{table}[!htb]
\small
\centering
\caption{Effect of reset on median per device cumulative download (GB) and median time Co-Bandit takes to stabilize (whether at Nash equilibrium or some other state).}
\label{table:minimal_reset_cumulative_download_stabilization_rate}
\newcolumntype{L}{>{\centering\arraybackslash}p{2.22cm}}
\begin{tabular}{l L L}
\hline
\textbf{Algorithm} & \textbf{Cumulative download (GB)} & \textbf{\# time slots to stabilize} \\ \hline
\multicolumn{1}{l}{\textbf{Co-Bandit}} & 6.87 & 175 \\ 
\multicolumn{1}{l}{\textbf{Co-Bandit with reset}} & 6.90 & 587 \\ 
\multicolumn{1}{l}{\textbf{Smart EXP3}} & 3.44 & -
% 1008 
\\ 
\hline
\end{tabular}
\end{table}
